Revealing the nanogeometry of WS2 nanoflowers by polarization-resolved Raman spectroscopy

Recent studies of Transition Metal Dichalcogenides (TMDs) have revealed exciting optical properties like stable excitons and chiral light-matter interactions. Chemical vapor deposition (CVD) techniques provide a platform for the fabrication of nanostructures with diverse geometries, ranging from horizontal flakes to flower-like structures. Raman spectroscopy is commonly used to characterize TMDs and their properties. Here, we use polarization-resolved Raman spectroscopy to probe the nanogeometry and orientation of WS2 nanoflower petals. Exciting the nanoflowers with linearly polarized light, we observe an enhanced Raman response from flower petals oriented along the excitation polarization direction. Furthermore, the helicity-resolved Raman response of vertically oriented wall-like flower petals exhibits clear differences with horizontally oriented flakes. Although the photoluminescence from the nanoflowers is strongly reduced, the Raman response upon excitation in resonance with the WS2 excitonic transition does reveal the presence of the exciton, which results in a distinct temperature dependence of the Raman response.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
